A Federated CloudNet Architecture: The PIP and the VNP Role

We present a generic and flexible architecture to realize CloudNets: virtual networks connecting cloud resources with resource guarantees. Our architecture is federated and supports different (and maybe even competing) economical roles, by providing explicit negotiation and provisioning interfaces. Contract-based interactions and a resource description language that allows for aggregation and abstraction, preserve the different roles' autonomy without sacrificing flexibility. Moreover, since our CloudNet architecture is plugin based, essentially all cloud operating systems (e.g., OpenStack) or link technologies (e.g., VLANs, OpenFlow, VPLS) can be used within the framework. This paper describes two roles in more detail: The Physical Infrastructure Providers (PIP) which own the substrate network and resources, and the Virtual Network Providers (VNP) which can act as resource and CloudNet brokers and resellers. Both roles are fully implemented in our wide-area prototype that spans remote sites and resources.

==> implementation.tex <==

\begin{comment}
\section{Anatomy of the CloudNets Architecture}

This section gives a ``big picture'', general overview of the CloudNets
Architecture. It will discuss the most important concepts and components and
how they add up to the greater whole of the CloudNets Architecture and its
implementation the Virtu Prototype.

\begin{figure}[t]
\centering
\includegraphics[width=.9\columnwidth]{architecture.pdf}\\
\caption{Key components of the CloudNets Architecture and their functions.}
\label{fig:architecture}
% TODO: not referenced in the text, yet
\end{figure}

\subsection{Describing and Exploiting Flexibilities}

The decoupling of services from the infrastructure greatly improves the
flexibility of networks. In a virtualized environment, the locations where a
CloudNet is realized (i.e., \emph{embedded}) is only constrained by the
CloudNet specification itself, i.e., the restrictions the CloudNet user (or
customer) imposes.

We deem it unlikely that a user specifies each and every detail of the
CloudNet; rather, specifications may often be \emph{vague} or absent entirely.
For example, a CloudNet used to out-source resources at peak times, may only
specify that the used cloud resources lie within \emph{Europe}, and e.g., a
Swiss or a British cloud provider may be chosen. Similarly, a CloudNet may not
specify which virtualization technology is used, or simply constrain it to Xen
virtualization without specifying specific kernel versions. A CloudNet can also
be delay-tolerant, e.g., a CloudNet for bulk data transfers.

This flexibility in the specification can be exploited for optimizations, for
instance by choosing the cheapest cloud provider, or by determining the
realization period where the load on the infrastructure is low or where
electricity is cheap. Within the limitations of the specification, a CloudNet
can also be \emph{migrated}.  A CloudNet provider can use migration to
co-locate CloudNets in times of low demand, to save energy if the remaining
network components can be switched off, or to perform maintenance work.

\subsubsection{Resource Description with Vagueness Support}


\subsubsection{Embedding and Service Migration}

There exist many algorithmic tools to exploit flexibility (see, e.g.,
%~\cite{onstrat11iptcomm,podccloud,infocom2009,icdcn12stefan,ammar,infocom12,zhu06},
%and especially the surveys
~\cite{alloc-survey,chalsurvey}).  We propose a \emph{two stage embedding}
approach: First, a CloudNet is embedded fast but heuristically. The resulting
embeddings can be suboptimal and resources are reserved on each physical
component (both nodes and links) to facilitate such quick placements.
Subsequently, the embedding of existing CloudNets is optimized in the
background according to a generic mathematical program (technically a
\emph{Mixed Integer Program}, short \emph{MIP}).\footnote{Optimizing long-lived
CloudNets is useful if CloudNet durations are heavy-tailed.} In the remainder
of this article, we will not discuss the heuristic embedding further but refer
the reader to the survey~\cite{virsurvey} on similar heuristics. Moreover, in
order to focus on the technical aspects, we do not describe the MIP used in our
prototype formally, but refer the reader to~\cite{grsch-tr} for details.

The mathematical programming approach is attractive as it is very general and
allows us to specify many different types of embeddings and embedding
constraints. For instance, while data center topologies are typically
relatively homogenous, embeddings on arbitrary Internet infrastructures with
heterogeneous resources and links requires a high flexibility. Our Mixed
Integer Program supports the mapping of full-duplex links on a set of
asymmetric links or broadcast links with multiple endpoints. It also
facilitates a simple replacement of the optimization function, without the need
to redesign the embedding algorithm. (Rather, the state-of-the-art and
optimized algorithms and heuristics provided by standard solvers such as
\emph{CPLEX} or \emph{Gurobi} can be used.\footnote{See
\texttt{http://www.cplex.com/} and \texttt{http://www.gurobi.com/}.})
For instance, one possible objective function may arise in
scenarios where a CloudNet should be embedded in such a manner that the maximal
\emph{load} or \emph{congestion} is minimized. In other scenarios, the
CloudNets should be embedded in a compact manner in order to be able to shut
down the other parts of the physical network, e.g., to save \emph{energy}.

Moreover, our architecture supports the live modification of - partial or whole -
CloudNets: As the CloudNet requests arriving over time may be hard to predict,
certain embeddings computed online in the past may become suboptimal, and
re-embeddings and migrations are necessary. Another reason for modifications is
network or server maintenance: in order to upgrade the infrastructure, it can
be useful to temporarily migrate (parts of) the network or the servers to an
alternative location.  While today's network virtualization technology
allows for seamless migration (without session interruption or address
reconfigurations), migration also comes at a cost (e.g., in terms of
computation, bandwidth, or even roaming fees in case of cross-provider
migrations). Whether and where to migrate is hence a non-trivial problem.

Many other special embedding requirements can be specified in the mathematical
program. E.g., the MIP supports embeddings across resources and resource types
(e.g., mapping storage to RAM and/or disk), and exact solutions for the mapping
of partial networks to single substrate nodes; it further allows providers to
formulate placement policies as well as resource priorities (e.g., prioritizing
lucrative resource allocations). Also node-based loads can be taken into
account, e.g., depending on the packet rate (shorter packets increase the
computational load at the forwarding engine), and so on.

By computing the embedding that would result after a migration together with
the migration cost, the MIP allows us to determine, e.g., the
\emph{cost-benefit tradeoff} of migration. For example, our algorithm allows to
answer questions such as: Can we migrate CloudNets to a more compact form such
that 20\% of the currently used resources are freed up, and what would be the
corresponding migration cost? It is then left to the (potentially automated)
administrator to decide whether the changes are worthwhile.

\subsection{Hierarchical Tree Of Roles: Distributing The Embedding Problem}

One key advantage --- or side effect --- of vagueness support and federated
roles is an automatic distributed computation of the mapping problem: While
full computation for a large topology graph may be infeasibly expensive for any
one player the hierarchical architecture will naturally distribute the load:
High level roles such as the VNO (that do operate on a CloudNet's full topology
graph) will only have to compute a fairly simple allocation that maps partial
graphs to a small number of lower-rung players. In addition vagueness support
helps in keeping higher level roles' computations simple, since Features and
Resources said high-level roles do not care about (and which are at the
lower-rung players' discretion) need not be taken into account at this level.

\subsection{Plugin Based Architecture}

Much like Ericsson's Network Embedded Cloud \cite{ericsson2} the CloudNets
architecture is plugin-based to faciliate extensions and adaptations to new
networking and virtualization technologies. Plugin-based operation hinges on a
feature of the RDL, typed NetworkElements:

The \emph{NetworkElement}  objects of the Resource Description Language all
have a hierarchical \emph{attribute} field (this also applies to the
\emph{NetworkInterface}, \emph{Resource} and \emph{Feature} objects). This
field is a string of hierarchy levels separated by forward slashes, much like a
path in a Unix file system (e.g.  \texttt{/node/host/generic}).

Much like a CloudNet, any player's substrate can be described in terms of the
RDL. Hence all substrate elements will have an \emph{attribute} field. Once a
CloudNet's resources have been mapped to a player's substrate resources this field
will be used to determine which plugin to use to embed the NetworkElement in
question.  Depending on the substrate NetworkElement's hardware --- or software
--- (e.g.  Layer 2 VPNs, Ethernet, MPLS, Mainframes, VM hosts) the appropriate
embedding plugin can be chosen to embed all the CloudNet's resources mapped to
the substrate element in question.

\subsection{Beyond Network Virtualization: Resource Allocation Outside Networking}

Since operations on concrete hardware or software --- or indeed the very
mention of concrete hardware or software --- only takes place as late as a
specific embedding plugin being invoked the CloudNets architecture could
readily be adapted for resource allocation well outside the networking domain:

Given suitable embedding plugins it could be used to optimize global logistics
(e.g. by mapping containers or other types of cargo to warehouses linked by
shipping lanes), road traffic (e.g. by mapping certain destinations to
intersections and routes through a city and implementing an embedding plugin
for a \texttt{/node/billboard/electronic} NetworkElement) or for handling power
transmission in a smart grid (by mapping localized peaks or lows in production
to a substrate of power consumers connected by the smart grid).

\end{comment}

\section{The CloudNets Prototype}\label{sec:prototype}

The CloudNets prototype is a proof-of-concept implementation of the architecture described above.
Currently, the prototype implements the PIP
business role (the infrastructure provider) as well as the VNP business role
(the resource broker). As a link virtualization plugin we use \emph{tagged VLANs}: each virtual
link is realized as a VLAN. The VLANs provide isolation and facilitate the
demultiplexing of the packets to the corresponding virtual machines (to which
the connection looks like an Ethernet link).

In the following, we will first give an overview of the testbed and then
discuss the prototype. In the context of the prototype, we will refer to
virtual nodes as \emph{VNodes} and to virtual links as \emph{VLinks}. Moreover,
we will distinguish between the \emph{mapping} of a CloudNet (i.e., where to
allocate the CloudNet in the substrate) and the \emph{embedding} of a CloudNet
(the actual implementation of said allocation).

\subsection{Testbed}

\begin{figure*}[t]
\centering
\includegraphics[width=.85\textwidth]{testbed.pdf}\\
\caption{Overview diagram of a test topology for VNP level operations, spanning
both the TU Berlin and Docomo test beds. Note the physical substrate node
SN113 (loadgen121) that is also serving as a host for virtualized substrate
nodes.}
\label{fig:testbed}
\end{figure*}

Our network virtualization prototype is run on two separate testbed
environments (see Figure~\ref{fig:testbed} for an overview of the available
substrate nodes), one at TU Berlin (the \emph{Routerlab}) and
one at NTT DoCoMo Eurolabs, Munich. Both testbeds have a Cisco 4500 series
switch carrying both virtual network \emph{data plane} VLANs and \emph{testbed
management} VLANs. Moreover, both testbeds consist of Sun X4150 machines hosting both
substrate resources and the virtual machines running the various roles'
management software. Since there are not enough physical nodes available in the
\emph{Routerlab}, some substrate nodes are KVM virtual machines hosted on one
physical node. In the testbed in Munich there are more physical machines
available, hence every substrate node is a dedicated physical machine, with the
provider management nodes being virtual machines hosted on one physical
machine. Substrate nodes, management nodes and virtual nodes run Linux
(\texttt{Ubuntu 8.04}). Virtual can nodes either be fully virtualized
\emph{KVM} virtual machines where physical substrate nodes are available, or
paravirtualized \emph{Xen} virtual machines.

The substrate resource allocation for the CloudNet embeddings (CPU and memory
resources on virtual machine hosts, and network links for connections) is
computed with an optimized \emph{Mixed Integer Program (MIP)}. Once the   % jgr: Probably move this to the Anatomy section
resource allocation is determined, the physical infrastructure provider creates
virtual machines, establishes the links between them and hands control over to
the customer (by providing console access to the virtual nodes for instance).

At the heart of the prototype lie MySQL databases where each provider keeps all
information about its substrate topology and embedded virtual networks.  The
database holds a representation of the substrate topology (the \emph{Underlay
(UL) graph}, and for each embedded virtual network there is an \emph{Overlay (OL) graph}
describing the virtual network topology and a \emph{Mapping Layer (ML) graph}
describing the locations of the virtual network's components on the substrate
hosting them.


\begin{figure}[t]
\centering
\includegraphics[width=.9\columnwidth]{architecture_implemented.pdf}\\
\caption{The CloudNets Architecture as implemented by the Physical Infrastructure Provider role.}
\label{fig:architecture-impl}
\end{figure}


%\subsection{The PIP Level}

%TODO: function, challenges, implementation

%\subsection{The VNP Level}

\subsection{The Embedding Plugin}

%shows the CloudNets architecture as implemented in the Prototype.

In order to embed CloudNets on the given substrate topology, we pursue a mathematical programming approach and use a \emph{Mixed Integer Program} plugin (short \emph{MIP}). Currently, this is the only implemented embedding plugin in the prototype, but we are working on a fast alternative for the first embedding stage (see the discussion in Section~\ref{ssec:emb}). In order to focus on the technical aspects, we do not describe the used MIP in full detail, but refer the reader to~\cite{grsch-tr}.

The mathematical programming approach is attractive as it is very general and allows us to specify many different types of embeddings and embedding constraints. For instance, while data center topologies are typically relatively homogenous, embeddings on arbitrary Internet infrastructures with heterogeneous resources and links requires a high flexibility. Our Mixed Integer Program supports the mapping of full-duplex links
on a set of asymmetric links or broadcast links with multiple endpoints. It also facilitates a simple replacement of the optimization function, without the need to redesign the embedding algorithm. (Rather, the state-of-the-art and optimized algorithms and heuristics provided by standard solvers such as \emph{CPLEX}~\cite{cplex} or \emph{Gurobi}~\cite{gurobi} can be used.)
For instance, one possible objective function may arise in
scenarios where a CloudNet should be embedded in such a manner that the
maximal \emph{load} or \emph{congestion} is minimized. In other scenarios, the
CloudNets should be embedded in a compact manner in order to be
able to shut down the other parts of the physical network, e.g., to
save \emph{energy}.

Moreover, our MIP plugin also supports the migration of (parts of) a CloudNet:
As the CloudNet requests arriving over time may be hard to
predict, certain embeddings computed online in the past may become
suboptimal, and re-embeddings and migrations are necessary. Another
reason for migration is network or server maintenance: in order to
upgrade the infrastructure, it can be useful to temporarily migrate
(parts of) the network or the servers to an alternative location.
While today's network virtualization technology facilitates seamless
migration (without session interruption or address reconfigurations), migration also comes at a cost
(e.g., in terms of computation, bandwidth, or even roaming fees in
case of cross-provider migrations). Whether and where to migrate is
hence a non-trivial problem.

Many other special embedding requirements can be specified in the mathematical
program. E.g., the MIP supports embeddings across resources and resource types (e.g., mapping storage to RAM and/or disk), and exact
solutions for the mapping of partial networks to single substrate
nodes; it further allows providers to formulate placement policies as well as
resource priorities (e.g., prioritizing lucrative resource
allocations). Also node-based
loads can be taken into account, e.g., depending on the packet rate (shorter packets
increase the computational load at the forwarding engine), and so on.

By computing the embedding that would result
after a migration together with the migration cost, the MIP allows us to determine, e.g., the
\emph{cost-benefit tradeoff} of migration. For example, our algorithm allows to answer
questions such as: Can we migrate CloudNets to a more compact form
such that 20\% of the currently used resources are freed up, and
what would be the corresponding migration cost? It is then left to the
(potentially automated) administrator to decide whether the changes
are worthwhile.

\subsection{PIP and VNP Roles}

In the following, we will focus on the two main roles in our architecture, the
\emph{PIP (Physical Infrastructure Provider)} and the \emph{VNP (Virtual
Network Provider)}, and describe their implementation in the prototype.

\subsubsection{Graph Serialization}

A first and important task to be solved to permit role interactions is
\emph{graph serialization}.  Since the management nodes for the VNP and the
PIPs in its substrate graph all run on dedicated machines with dedicated
databases, graphs representing the CloudNet topologies have to be serialized
into a database independent representation to be sent across the network. To
this end we developed a \emph{YAML}~\cite{yaml} representation of the resource description
language, along with serialization/deserialization mechanisms to convert the
database representation of a graph into a format suitable for transmission and
back into a database representation on the other side.

\subsubsection{The PIP}

The PIP role supports arbitrary topology specification and topology
modification including live migration of running nodes (within a PIP's % TODO jgr: Have a look at Ericsson paper again, figure out exactly _how_ uncommon online topology modification is
substrate). Its main components are the \emph{Mapping Component} that handles
the Mixed Integer Program formulation, result interpretation and Mapping Layer
graph generation, and an extensible (plugin based) \emph{Embedding Component}
that embeds a (partial) CloudNet topology on the PIP's substrate given its
overlay and mapping layer graphs. Figure~\ref{fig:architecture-impl} gives an
overview of these components.

\paragraph{Substrate}

The PIP's substrate is largely virtualized in our testbed in Berlin: most substrate
nodes are KVM virtual machines running on the testbed's Sun X4150 machines.
The X4150s are interconnected by an \texttt{IEEE
802.1q}-capable
switch. The virtualized substrate nodes are assigned unique Ethernet addresses
and connected via physical Ethernet interfaces. The CloudNet VNodes are then
created on said KVM virtual machines. Each virtual link is assigned a unique
VLAN tag (picked by the PIP from its assigned range of VLAN tags). These VLAN
tags are set on all data plane interfaces (or switch ports) with substrate
nodes participating in the virtual link.

In addition to this some of the X4150 machines are configured to serve as
substrate nodes themselves, on top of hosting virtualized substrate nodes. They
can host fully virtualized KVM VNodes (as opposed to the virtualized substrate
nodes which can only host paravirtualized Xen SNodes).

All substrate nodes store their VM images on an NFS share exported by their
controlling PIP. PIPs are responsible for creating VM images and hypervisor
configurations, while the substrate nodes' provisioning scripts take care of
the rest.

Interconnections between links that do not involve VNodes are realized by
creating bridge devices on dedicated \texttt{Tunnel Bridge (TBR)}
nodes. Unlike regular substrate nodes these do not run OpenVSwitch but the
regular Linux bridge.\footnote{This is mostly due to historical reasons: some functionality
(mainly bridging between different VLANs) was required on these nodes - which
was not supported by \emph{OpenVSwitch} (\texttt{http://openvswitch.org/}) at
the time.} They can host virtual switches and
terminate OpenVPN tunnels. In particular these bridge devices are used to
establish VLinks spanning across PIP boundaries (\emph{transit links}):
They interconnect the outside segment of these links (within the specifying
VNP's management scope) with the internal segment of these links (within the
PIP's management scope). The mechanism behind this is based on OpenVPN TAP
style layer two tunnels: These are VPN tunnels terminating in virtual ethernet
devices on both tunnel bridges involved in the transit link. Said virtual
interfaces trunk all VLinks embedded on the transit link in question and are
bridged to the tunnel bridges' data plane interface.

\paragraph{Cloud Operating System Functionality}

Since Cloud Operating Systems such as OpenStack were still in their infancy
when the prototype was developed, the prototype provides some of the same
services modern Cloud Operating Systems provide (or plan to provide):

\textbf{Automated VM Provisioning.}
The Embedding Component automatically creates VM images for VNodes (typically
by making copies of a template VM image suitable for the hosting substrate
node's hypervisor) and hypervisor configuration files. With everything in place
these VMs can be started through an XMLRPC interface to the hosting substrate
node's provisioning scripts. This interface offers a range of basic VM
provisioning functionalities such as \emph{start}, \emph{stop}, and
\emph{powercycle}.

\textbf{VM Image Caching.\label{clipd}}
Since the I/O performance of the X4150 machines is rather poor and there is
plenty of storage space available we developed a caching scheme to speed up
CloudNet embedding. There is a daemon, \emph{clipd}, that maintains a cache of
VM images on every PIP's exported NFS share (on disk). The Embedding component can
request VM images from this daemon's cache, which are then be moved to their
final location on the NFS share, thus greatly speeding up the whole embedding
process. The \emph{clipd} cache is replenished by a cron job while the Mapping
Layer/Embedding is inactive.

\textbf{Customer Console Access to VNodes.}
Since placement of VNodes is rather opaque to a PIP's customers --- and not
relevant as long as their requirements are met --- there is a mechanism to
automatically look up any given VNode's hosting substrate node, and offer a
proxied serial console session on that very VNode to a customer requesting
access.

\textbf{Automated Link Provisioning.}
Virtual links are provisioned and brought up automatically. In the Mapping
Layer graph they are split up into segments, one for each substrate network
element they are mapped to (for instance the two substrate nodes on either end
and the switch port the substrate nodes' data plane interfaces are connected
to). For each of these components appropriate Embedding Plugin is called. To
date there are Embedding Plugins handling OpenVSwitch based hosts, traditional
Linux Bridge based hosts and Cisco 4500 series switches (the latter are
configured via SNMP).

\begin{figure}
\centering
\includegraphics[width=.9\columnwidth]{negotiation_interface.pdf}\\
\caption{Interfaces between roles in our prototype.}
\label{negotiation-if}
\end{figure}

\paragraph{Negotiation and Provisioning Interface}

A PIP controls its substrate nodes and (physical) switch through an
\emph{XMLRPC}~\cite{xmlrpc} configuration interface. The PIP in turn
offers two interfaces to the VNP role: The \emph{Negotiation Interface} and the
\emph{Provisioning Interface} (see Figure~\ref{negotiation-if} for an overview
of interfaces between roles). Both consist of a range
of \emph{XMLRPC} methods.

Negotiation follows a two-stage protocol: The Negotiation Interface allows
for sending preliminary embedding requests for either topology creation or
modification of previously embedded topologies. Once a VNP is sure it wants to
embed a topology (i.e., after receiving the `okays' from all involved PIPs), it
will send a confirmation request for the preliminary topology.

The VNodes of an embedded topology can then be started and stopped through the
Provisioning Interface.

\subsubsection{The VNP}

The VNP's high-level architecture is similar to the PIP's, also comprising a
Mapping Component and an Embedding Component. The Mapping Component is for the
most part identical to the PIP's. The major differences are in the embedding
component: (1) since the VNP's substrate consists of entire PIPs rather than
physical nodes and links, the VNP has its own set of embedding plugins to
interact with PIPs' Negotiation Interfaces; (2) the Embedding Component
contains additional code for the creation of \emph{partial graphs} which can be
mapped to a single PIP.

\paragraph{Substrate}

The VNP's substrate consists of PIP nodes interconnected by \emph{transit
links}\footnote{In our prototype, these are represented by \emph{OpenVPN} (see
\texttt{http://openvpn.net/}) \texttt{tap} style tunnels between the PIPs'
tunnel bridge nodes.}. Hence the VNP is aware of the topology between PIPs (or
a subset of said topology) but does not know anything about the PIP's internal
topology.

\paragraph{Negotiation and Provisioning Interface}

A library on the VNP level implements the client side functionality of the
PIP's Negotiation and Provisioning Interface. It is used to send partial
topology graphs to PIPs and embed them.

\subsection{Life of a CloudNet Request}\label{ssec:life}

\begin{figure}
\centering
\includegraphics[width=.9\columnwidth]{data_flow.pdf}\\
\caption{Stages of a CloudNet request from VNP to PIP.}
\label{stages}
\end{figure}

In order to illustrate the operation of our prototype, we describe the
processing stages a CloudNet topology request graph undergoes from initial
submission to the VNP to final embedding of all its nodes on one or multiple PIPs.
See Figure~\ref{stages} for a graphical outline of these stages.

\subsubsection{Incoming CloudNet Request}

The CloudNet request in the form of an `overlay graph' (henceforth referred to
as \emph{OL0 graph}) is submitted to the VNP (as a serialized topology graph,
through an XMLRPC interface similar to the PIP's Negotiation Interface).
Subsequently, the VNP's mapping process is started.

\subsubsection{Substrate Synchronization}

The first step in mapping a CloudNet request is substrate synchronization: The VNP
uses the Negotiation Interface to update the available resources on the PIPs in its
substrate. Currently, our prototype supports RAM only, and to give the VNP a rough
approximation of a given PIP's available resources, we simply sum up all the
resources in the PIP's substrate (i.e., a PIP with three substrate nodes that have
4GB RAM each will report an aggregate resource of 12GB RAM to the VNP).

\subsubsection{Solution of VNP-level MIP and ML Graph Generation}

Before proceeding with the mapping process proper, the VNP completes the OL0
graph, yielding an \emph{OL1 graph}. This is to account for any vagueness on
the upstream entity's part (i.e. values are chosen for those required resources
and features that were left unspecified; for instance the virtualization
technology might not have been specified, allowing the VNP to make a choice of
its own or pass the the vague graph on to downstream players, who will in turn
have the freedom of choice). Next it formulates the Mixed Integer Program (MIP)
for mapping the incoming CloudNet request to its substrate of PIPs. The MIP is
based upon the following variables:
(1) the incoming OL0 graph's resource and feature requirements and constraints,
(2) the available resources and features on the PIPs constituting the VNP's substrate (as far as they are known to the VNP), and
(3) the available resources and features on the transit links between PIPs.

Once the MIP has been solved the result is translated back into a mapping layer
graph, mapping all of the OL1 graph's Network Elements (NEs) to PIPs and transit
links.

\subsubsection{Partial Graph Generation}

Now the VNP iterates through the OL1 graph and creates a set of partial graphs,
one for each PIP. Each of these partial graphs consists of all the NEs mapped
to the PIP in question.

In the course of partial graph generation, stubs for transit links are created.
These consist of two special network element types: \texttt{/node/host/pip} and
\texttt{/link/transit}.

The \texttt{/link/transit} \emph{NE} specifies the VLAN to use for this transit link
(we opted for letting the VNP pick transit VLANs to avoid implementing an error
prone PIP-to-PIP negotiation mechanism for this purpose). This closely matches
the most likely real-world scenario, too: A VNP might have an embed plugin for a
transit provider (for instance someone running a MPLS network) with black boxes
located at both PIPs' network edges. This embed plugin requests a transit link
between these two PIPs and receives some kind of link identifier (such as a
VLAN tag). The VNP then communicates this link identifier to the PIPs on either
end, which allows both PIPs to connect the black box to their local segment of
the virtual link.

The \texttt{/node/host/pip} allows for some vagueness in the VNP's substrate
graph (and flexibility for the PIP) since it tells the PIP which other PIP the
transit link is supposed to connect to. As long as the bandwidth requirements of the VNP are
fulfilled, the PIP is free to assign the corresponding resources.

\subsubsection{Partial Graph Serialization and Transmission to PIPs}

Once the partial graphs have been assembled, each of them is serialized and
sent to its hosting PIP through the Negotiation Interface. This currently takes
place in a serial manner in our prototype, i.e., partial graphs are sent to PIPs one after the
other. If one of the PIPs in the chain turns out to be unable to embed its
partial graph the VNP rolls back the already embedded partial graphs (deletes
them) and reports a failure status to the upstream entity that sent the
original CloudNet request.

\subsubsection{Formulation and Solution of MIPs for Incoming Partial Graphs}

Upon receipt of a partial graph a PIP will---much like the VNP--- complete the
OL0 graphs to yield OL1 graphs, and formulate the MIP for mapping the incoming
partial CloudNet request to its substrate of physical hardware. The program is
based on the following variables:
(1) the incoming partial graph's resource and feature requirements and constraints,
(2) the available resources and features on this PIP, and
(3) the available resources and features on this PIP's outgoing transit links leading to requested destinations.

Once the MIP has been solved the result is translated back into a mapping layer
graph, mapping all of the OL1 graph's Network Elements to substrate links
and nodes. Control passes to the Embedding Component now which will configure
the topology's VLANs on the switch as specified by the Mapping Component and
create the VNodes' images and hypervisor configuration. With everything in
place the PIP reports success to the VNP who sent the (partial) CloudNet creation
request.

\subsubsection{VNode Bootup and Handoff to Customer}

Once success has been reported back to the VNP by all PIPs involved in the CloudNet
creation request, the VNP uses the PIPs' Provisioning Interface to
start the newly created VNodes (the links will already have been brought up in
the course of negotiation). Finally, the VNP hands control over the CloudNet to the
requesting upstream entity (typically in the form of console interfaces).

\subsection{Outlook}

 Our proof-of-concept prototype is optimized for flexibility and generality rather than performance.
 Although it is already fully functional, several extensions are planned.

\subsubsection{Inter-PIP Migration}

Currently, our prototype only supports migrations within a PIP. To enable VNode
migration across PIP boundaries, a mechanism is required that orchestrates
migration on the VNP side and makes sure space for migrating VNodes is
allocated and ready before migration. This implies slight modifications to the
negotiation and provisioning interfaces and some changes to the PIP's embedding
component.

On the substrate side we are currently evaluating the following synchronization
mechanisms for migration:

\paragraph{Suspend and synchronize}

The simplest approach would be to suspend running VMs, synchronize their
disk images and then restore them. This is an approach that has been used
before~\cite{azoff} and would hold the advantage of being hypervisor agnostic
and easy to implement --- at the possible cost of some efficiency.

\paragraph{DRBD backed VM images}

Slightly more involved than the previous method this is based on using
DRBD~\cite{drbd} volumes as storage backend for VM images. They behave like
regular block devices from the VM's perspective and can be mirrored across a
network, with the possibility to attach a mirrored device online. A drawback of
this approach is the possibility for
deadlocks\footnote{\texttt{http://www.drbd.org/users-guide/ch-configure.html}}
if the DRBD volumes reside on a loop device.

\paragraph{Xen Live Migration}

Last but not least, recent Xen~\cite{xen-project} versions include a migration
mechanism that does not depend on VM images residing on shared storage. This
option is the least favoured one, since unlike the other two it is not
hypervisor agnostic and hence requires another mechanism for substrate nodes
that use a different hypervisor.

\subsubsection{Asynchronous and Parallel Operation}

As mentioned in Section~\ref{ssec:life}, negotiations with PIPs
currently take
place in a serial manner. Yet it would be desirable to negotiate with all
involved PIPs in parallel, thus exploiting the distributed nature of the
architecture. Likewise it would be desirable to decouple mapping and embedding:
Currently preliminary graphs are simply embedded and deleted after a certain
amount of time has passed without a confirmation arriving. Decoupling mapping
and embedding would hold the following advantages:

\begin{itemize}
\item No embedding overhead for preliminary graphs that are not
embedded eventually. Additionally, this would allow for quasi-parallel operation
without major changes at the VNP level: VNPs would only have to wait for each PIP's
mapping step to run to completion rather than for the embedding step.\footnote{In the
small topologies used for prototype development and testing, embedding takes
about five minutes, as opposed to about 20 seconds for the mapping.}

\item It would become possible for the VNP to request new mappings that entail VNode
migration without actually changing the currently embedded CloudNets on any PIP.
Hence the VNP could request mappings from all involved VNPs, migrate the nodes
that would end up on different PIPs, and only then confirm its requests,
effecting the rest of the changes.
\end{itemize}

\subsubsection{Terminal Attachment}

Eventually, we also need to address the problem of \emph{terminal attachment}
and develop a mechanism for attaching clients to CloudNets. We are currently
envisioning a role that presents itself as a PIP on the CloudNet side with a
special \emph{customers} resource that contains the number of currently
connected terminals. Thus, scenarios such as a Service Provider specifying
CloudNet requirements like ``My service must reach 20k or more terminals!'' or
``My service must reach all Swiss users at a latency below 20ms!'' are % jgr: Expressing "all Swiss citizens" in the RDL is rather difficult
supported.

%\begin{figure}
%\centering
%\includegraphics[width=.6\columnwidth]{13nodes.pdf}\\
%\caption{\texttt{13nodes}: Sample topology used in evaluating VNP performance}
%\label{fig:13nodes}
%\end{figure}


\begin{table}
\label{table:avgs}
\centering

\begin{tabular}{lcccc}
\textbf{VNP processing time:} & & & \\
& \textbf{Overall} & \textbf{Without VNP MIP} & \textbf{MIP duration} \\
\textbf{Mean:} & $722s$ & $721s$ & $1s$ \\
\textbf{Standard deviation:} & $2s$ & $2s$  & $0s$ \\
\hline
\textbf{PIP processing time:} & & & \\
\textbf{(without clipd)} & & & \\
& \textbf{PIP1} & \textbf{PIP2} & \textbf{Both PIPs} \\
\textbf{Mean:} & $631s$ & $27s$ & $659s$ \\
\textbf{Standard deviation:} & $18s$ & $1s$  & $20s$ \\   %
\hline
\textbf{Overhead} & & & \\
& & & \\
\textbf{Mean:} & $62s$ & & \\
\textbf{Standard deviation:} & $17s$ & & \\
\hline
\textbf{PIP processing time:} & & & \\
\textbf{(with clipd)} & & & \\
& \textbf{PIP1} & \textbf{PIP2} &  \\
\textbf{Mean:} & $123s$ & $14s$ & \\
\textbf{Standard deviation:} & $90s$ & $0s$  & \\   %
\hline
\end{tabular}
\caption{Average durations and standard deviations (over 50 repetitions) for various steps in embedding a sample star topology with 13 nodes.}\label{tab:times}
\end{table}

\subsubsection{Performance}

Table~\ref{tab:times} provides a first look at the performance of the currently
unoptimized prototype. We studied a scenario where the VNP embeds a CloudNet
with 13 nodes arranged as a star topology on two PIPs. The CloudNet is too
large for a single PIP, and hence twelve VNodes are placed on PIP1 and one
VNode on PIP2. We measured the time spent in total on the VNP and on the two
involved PIPs. Our results indicate that especially the VNP level processing
may be optimized further, as on average $62s$ are spent outside the MIP
computation. Also, we find that copying the virtual nodes entails relatively
high disk I/O costs with the slow RAID controllers used in our
testbed.\footnote{The LSI RAID controller exhibits a poor performance under
Linux and must be run in RAID0 mode to achieve reasonable disk performance.} We
have recently found that disk I/O performance can be significantly improved by
caching (see Section~\ref{clipd}) several VM images and moving them into place
on the PIPs' NFS exports as they are needed (as opposed to copying them). A
small scale test run (involving just the PIP level) has been conducted and
shows considerable improvement over prototype operation without \emph{clipd}.


\begin{comment}

\subsection{A Migration Demonstrator}

Besides the prototype itself, we also implemented a service migration
demonstrator which is used for demos at industrial partners, conferences and
science fairs.  Basically, the demonstrator consists of two parts: (1) a
\emph{topology demonstrator} which demonstrates how virtual networks
(CloudNets) are embedded in a given substrate network, and (2) a \emph{video
demonstrator} which demonstrates how a migrating streaming server can improve
QoS for the mobile terminals (the use case in this article).

The idea is that while the CloudNet can be placed anywhere in the substrate
network (e.g., a computational CloudNet without many user interactions), the
video server is a latency-sensitive service and should always be close to the
users. We set the resources (in our case: the RAM memory) in the demonstrator
in such a way that at any given time only one substrate node can accommodate
the streaming server in addition to the different CloudNet nodes hosted on the
shared substrate. Therefore, whenever the streaming server migrates (e.g., in a
``move-with-the-sun''' scenario), parts of the other CloudNets need to be moved
as well (moved ``against the sun'').

Figure~\ref{video-web} shows the web interface of our video demonstrator. It
allows the user to interactively add and remove clients from the access points,
causing the video server to migrate accordingly. The clients connected to the
access point hosting the video server receive the stream before the clients
attached elsewhere.\footnote{See also the demo at\\
\texttt{http://www.youtube.com/watch?v=llJce0F1zHQ}.} The topology demonstrator
web interface contains a list of three sample topologies, each with an {\em
embed} and a {\em delete} button. In addition there is a table showing all of
the PIP's currently embedded virtual nodes and the substrate nodes they are
hosted on.

\begin{figure}
\centering
\includegraphics[width=.2\columnwidth]{video-web.png}\\
%\includegraphics[width=.7\columnwidth]{topology-web.png}
\caption{Video Demonstrator web interface.}
\label{video-web}
\end{figure}

\subsubsection{Demonstrator Requirements}

The Topology Demonstrator is simple, and be basically just engineered its
resource usage such that the migration of the video streaming server will cause
a resource shortage at the destination, and the virtual nodes of the Topology
Demonstrator to be migrated away accordingly.\footnote{The \texttt{Ubuntu}
image requires roughly 256 MB (i.e., the nodes of the topology demonstrator and
the access point are roughly of this size as well) and
the streaming server roughly 512 MB.}

Fig.~\ref{topology-ram} shows an exemplary RAM resource distribution that forces
 migration when a virtual server migrates (the service virtual machine
is configured to take precedence over all other nodes).

\begin{figure}
\centering
\includegraphics[width=.2\columnwidth]{topology-ram.pdf}
\caption{Exemplary relative sizes of virtual nodes and substrate nodes in terms
of RAM. The single-letter nodes are virtual topology nodes. This describes a
forced migration scenario in the sense that no matter where the service VM
migrates to, at least one topology demonstrator node will have to migrate away
to make room.} \label{topology-ram}
\end{figure}

In the Video Demonstrator, the following challenges need to be addressed.
(1) \textbf{Client connectivity:} Streaming clients outside the testbed (and
hence outside the scope of CloudNet management) need to receive a video stream
from a virtual node, the streaming server, inside the video demonstrator's
virtual network. (Currently, our demonstrator does not support VLAN terminal
attachments.) (2) \textbf{Latency augmentation:} While the latency of local
(hosted on the same substrate node) versus remote (hosted on different access
points) clients is too small to have a detectable (to the human eye) impact on
a video stream, for the demonstration, we use a traffic engineering / buffering
mechanism that delays the video stream to remote clients to cause an artificial
delay in the video stream received by the clients.
(3) \textbf{Control of clients through the web interface:} Clients are
enabled/disabled through the web interface. Since the clients are not
accessible from the PIP management node the web interface runs on, an
indirection is required.
(4) \textbf{Virtual node control:} Latency augmentation likely requires
modification of the virtual node state (either access point virtual nodes or
the streaming server VM). To this end, we decided to implement a
non-interactive way to send commands to virtual node consoles.

The interaction of the two demonstrators poses several challenges. Since they
both modify the same database (by virtue of invoking the mapping layer) there
needs to be a synchronization mechanism that avoids concurrent (and potentially
conflicting) database writes. There is also a need for more than rudimentary
CloudNet modification functionality.

\subsubsection{Implementation}

The Video Demonstrator incorporates a range of backend scripts on the
infrastructure provider, some code running on the service virtual node, and a
multi-layered VPN tunnel architecture to connect the streaming clients to the
testbed.  A schematic overview is given in Figure~\ref{topology-ram}. It shows
the different static VLANs in use as well as the VLAN assigned automatically by
the mapping layer (ML).
\begin{figure}
\centering
 \includegraphics[width=.4\columnwidth]{topology-mono.pdf}
\caption{Video Demonstrator overview schematic. One VLAN connects all three
access points and the streaming server, and each triple of clients shares an
additional VLAN. The client VLANs are interconnected through a bridge by the
access points. Currently, the traffic shaping happens at the server (via
console access from the PIP), depending on the server position (client ports
are used to determine the required shaping). Access points are fixed and are
not migrated.}
\label{topology-ram}
\end{figure}

In the demonstrator, there are three {\em client machines}. Each client machine
runs three VLC instances in UDP listening mode that represent the clients
connected through the access point associated with this client machine. Each
client is associated with a unique client port. The server runs a VLC instance
for each client, each of which sends the same video stream to its assigned
client. Clients are enabled/disabled by inserting and removing
\texttt{iptables}\footnote{See \texttt{http://www.netfilter.org}.} rules that
pass or drop UDP traffic to the client's port. This does not cause any
disruption (such as clients timing out and giving up on the video stream after
extended periods of remaining disabled) since VLC's UDP based streaming
protocol is stateless.

%\begin{figure}
%\centering
%\includegraphics[width=.7\columnwidth]{client-architecture.pdf}
%\caption{VLC client architecture}
%\label{client-architecture}
%\end{figure}

Clients connect to the testbed via a OpenVPN\footnote{See
\texttt{http://www.openvpn.org}\nocite{openvpn}.} \texttt{tap} style tunnel.
This VPN tunnel provides layer 2 connectivity (i.e., it tunnels IEEE 802.3
frames over IP). It terminates in a tap device on each client machine and its
counterpart on the substrate node.

On the \emph{tunnel bridge}, \texttt{tbr1} the clients' \texttt{tap} devices are
bridged onto that machines' CloudNet data plane interface, \texttt{eth2}. Each
client machine/access point pair is assigned a dedicated VLAN tag. This VLAN
tag is set on the bridge device interconnecting this client machine's and the
tunnel bridge's CloudNet data plane interface.

A bridge device is used on each access point, interconnecting its
two interfaces, thus forwarding the packets incoming from its client to the
server side interface and vice versa.

%Since freshly created VNodes all start out with the same default system image,
%there default images are replaced by the demonstrator nodes' actual images. Finally, these virtual nodes are started. all virtual nodes run the
%same default system image, the actual system images
%for the access point and server virtual node are copied over as a last step over the default images and starts the
%virtual nodes.

When a client is added to an access point, the center of gravity of demand is
recomputed.\footnote{Concretely, the server is migrated to the access point
with the most clients. Ties are broken in favor of the leftmost access point.}
If the newly computed center of gravity differs from the center of gravity
recorded in the server state file it sends a migration request to the migration
daemon.  It will cause the mapping layer to replace the currently embedded
video demonstrator CloudNet topology by one that co-locates the server with the
new center of gravity.

\end{comment}

%\section{Use Case: OpenStack}\label{sec:openstack}
%
%Maybe describe how to integrate openstack architecture and wind etc. (ev. koennen wir dann ericsson schreiben dass wir uns mal ueberlegt haben wie wirs kombinieren %koennen, und bei der gelegenheit fragen ob sie interesse haben was zusammen zu machen?)

